Automatic Teller Machines for Offline E-cash

Electronic cash (e-cash) is a digital alternative to physical currency that allows anonymous transactions between users and merchants. Typically, coins in an e-cash scheme are only dispensed through a central bank. A drawback of this approach is that the bank is always on the critical path during withdrawals, and if a reliable connection to the bank is temporarily unavailable, users may be unable to withdraw coins in a timely fashion. As with physical currency, there are benefits to supporting a decentralized infrastructure where withdrawals can be performed without involving the bank in the critical path. We propose the design of a new cryptographic bearer token that can be dispensed by automatic teller machines (ATM) in a fully offline e-cash scheme. Such bearer tokens provide anonymity, unforgeability and untraceability, i.e., users cannot be tracked by their spending activities or the locations of withdrawal. We formalize the requirements of an e-cash scheme with multiple issuers and propose an efficient design building on top of the compact e-cash protocol of Camenisch et al. (EUROCRYPT 2005). Our construction leverages an unforgeable and doubly-anonymous voucher that allows a one-time transfer of coins between an ATM and a user, while hiding their identities from parties not involved in the transaction.

==> tables/related.tex <==
\begin{table}[t]
% \fontsize{5.6}{5.6} \selectfont
\scriptsize
% \tiny
\setlength{\tabcolsep}{2pt}
\caption{Comparison of privacy-preserving vehicular reputation systems.}
  \label{tab:related}
  \centering
  \makegapedcells
\begin{tabular}{| c | c | c | c | c | c |}
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
\multirow{2}{*}{\makecell[c]{\\System Name}} & \multirow{2}{*}{\makecell[c]{\\Who rates\\vehicles}} & \multicolumn{2}{c|}{Threat model} & \multicolumn{2}{c|}{Security/Privacy properties} \\
\cline{3-6}
& & \makecell[c]{Trusted\\party} & \makecell[c]{Vehicle local\\anonymity} & \makecell[c]{Unforge-\\ability} & \makecell[c]{Untraceability\\of RSU visit} \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
PPRU~\cite{liu2023ppru} & Vehicles & Servers & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \emptycirc[0.8ex] \\
\hline
RPRep~\cite{wang2016rprep} & Vehicles & Servers & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \emptycirc[0.8ex] \\
\hline
VRepChain~\cite{liu2022vrepchain} & Vehicles & \makecell[c]{Majority\\of RSUs} & \fullcirc[0.8ex] & \halfcirc[0.8ex] & \emptycirc[0.8ex] \\
\hline
Wang et. al.~\cite{wang2019rsu} & \makecell[c]{RSU/\\Server} & \makecell[c]{RSUs \&\\servers} & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \emptycirc[0.8ex] \\
\hline
\sys & RSU & N/A & \emptycirc[0.8ex] & \fullcirc[0.8ex] & \fullcirc[0.8ex] \\
\noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
\end{tabular}
\end{table}


% \begin{table*}[t]
% % \fontsize{5.6}{5.6} \selectfont
% \scriptsize
% % \tiny
% \setlength{\tabcolsep}{2pt}
% \caption{Comparison of state-of-the-art privacy-preserving vehicular reputation systems.}
%   \label{tab:related}
%   \centering
%   \makegapedcells
% \begin{tabular}{| c | c | c | c | c | c | c |}
% \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
% \multirow{2}{*}{System Name} & Application & \multicolumn{2}{c|}{Threat model} & \multicolumn{3}{c|}{Security/Privacy properties} \\
% \cline{3-7}
% & compatibility & Trusted party & Local anonymity of vehicles & Unforgeability & Untraceability of RSU visits & Responsiveness to misbehavior \\ % & Vehicle & RSU & Server & Vehicle-RSU & RSU-Server \\
% \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
% PPRU~\cite{liu2023ppru} & Vehicles rate vehicles & Servers & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \emptycirc[0.8ex] & \fullcirc[0.8ex] \\ % & $\sim 100$ & N/A & $\sim 10$ & $1-10$ & $1.5-10.5$ \\
% \hline
% RPRep~\cite{wang2016rprep} & Vehicles rate vehicles & Servers & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \emptycirc[0.8ex] & \fullcirc[0.8ex] \\
% \hline
% VRepChain~\cite{liu2022vrepchain} & Vehicles rate vehicles & A majority of RSUs & \fullcirc[0.8ex] & \halfcirc[0.8ex] & \emptycirc[0.8ex] & \halfcirc[0.8ex] \\
% \hline
% Wang et. al.~\cite{wang2019rsu} & RSU/Server rates vehicles & RSUs and servers & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \emptycirc[0.8ex] & \fullcirc[0.8ex] \\
% \hline
% \sys & RSU rates vehicles & N/A & \emptycirc[0.8ex] & \fullcirc[0.8ex] & \fullcirc[0.8ex] & \halfcirc[0.8ex] \\
% \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
% \end{tabular}
% \vspace{0.2em}
% \end{table*}

